CHATATC: Large Language Model-Driven Conversational Agents for Supporting Strategic Air Traffic Flow Management

Generative artificial intelligence (AI) and large language models (LLMs) have gained rapid popularity through publicly available tools such as ChatGPT. The adoption of LLMs for personal and professional use is fueled by the natural interactions between human users and computer applications such as ChatGPT, along with powerful summarization and text generation capabilities. Given the widespread use of such generative AI tools, in this work we investigate how these tools can be deployed in a non-safety critical, strategic traffic flow management setting. Specifically, we train an LLM, CHATATC, based on a large historical data set of Ground Delay Program (GDP) issuances, spanning 2000-2023 and consisting of over 80,000 GDP implementations, revisions, and cancellations. We test the query and response capabilities of CHATATC, documenting successes (e.g., providing correct GDP rates, durations, and reason) and shortcomings (e.g,. superlative questions). We also detail the design of a graphical user interface for future users to interact and collaborate with the CHATATC conversational agent.

==> ICRAT2024_schatATC/chapters/contributions.tex <==
% \section{Contributions of work}

% This paper represents the first exploration of using generative AI to help train new Air Traffic Managers and serve as a decision support tool for existing ones. Our contributions of work include:

% 2.	Scraping and summarizing 23 years of historical GDP data (which represents the most extensive GDP dataset of its kind)
% 3.	Training an LLM on a subset of the historical GDP data to create a fine-tuned prompt to answer questions about historical GDPs for specific airports
% 4.	Designing an interface prototype (i.e. ChatATC) for NTMO to interact with the trained LLM and ask it questions about historical GDPs
 
% 5.	Soliciting feedback from the NTMO regarding the interface prototype of ChatATC and exploring next steps to achieve implementation

